SimPropNet: Improved Similarity Propagation for Few-shot Image Segmentation

Few-shot segmentation (FSS) methods perform image segmentation for a particular object class in a target (query) image, using a small set of (support) image-mask pairs. Recent deep neural network based FSS methods leverage high-dimensional feature similarity between the foreground features of the support images and the query image features. In this work, we demonstrate gaps in the utilization of this similarity information in existing methods, and present a framework - SimPropNet, to bridge those gaps. We propose to jointly predict the support and query masks to force the support features to share characteristics with the query features. We also propose to utilize similarities in the background regions of the query and support images using a novel foreground-background attentive fusion mechanism. Our method achieves state-of-the-art results for one-shot and five-shot segmentation on the PASCAL-5i dataset. The paper includes detailed analysis and ablation studies for the proposed improvements and quantitative comparisons with contemporary methods.

==> src/experiments.tex <==
\section{Experimental Settings}



==> src/intro_new.tex <==
\section{Introduction}
\label{secIntro}
Semantic image segmentation assigns class labels to image pixels. It finds applications in image editing \cite{ Aksoy2, Aksoy1, SemanticSoftSeg, singa, Tai, Tan}, medical diagnosis \cite{HyperDenseNetAH, AttentionUL, UNet, MultiscaleGA}, automated driving \cite{Cordts_2016_CVPR} etc. Supervised deep neural network methods such as \cite{SegNet, dlv1, dlv2, DLV3, dlv3plus, DeepHR, psp} enable highly accurate image segmentation. However, they work for only a small number of fixed object classes, and require a large number of image-mask pairs for training which are hard to manually annotate. In several practical scenarios such as online commerce and design, obtaining dense annotations may be infeasible. Few-shot image segmentation methods, like \cite{OSLFSS, PANet, CANet}, are class-agnostic and alleviate the need for a large number of annotated images for each target object class. They use a small set of \textit{support} images and their segmentation masks for the target class as additional input to predict the segmentation mask of a given image. 
\begin{figure}[t]
\begin{center}
    \centering
    \includegraphics[width=0.9\linewidth]{src/images/FewshotSeg4.png}
\end{center}
\vspace{-4mm}
    \caption{Few-shot Image Segmentation: Broad architecture of contemporary methods (\cite{PANet, SGOne, CANet}). Features from the support image (in the support mask region) are processed to obtain a probe representation and fused with features from the query image, and decoded to predict the query mask. Improving similarity propagation between the support and query branches is the focus of this work. \vspace{-1mm}}
    \label{fig:task_seg}
\end{figure}
This work proposes a new network SimPropNet that significantly improves upon the state-of-the-art.

Few-shot segmentation (FSS) methods typically take as input - a \textit{query} image for which the segmentation mask is required, a set of \textit{support} images, and their segmentation masks (\textit{support masks}). One-shot segmentation is the extreme setting where only a single support image-mask pair is available. Our method achieves state-of-the-art performance in both one-shot and few-shot settings ($>$5\% and $>4$\% gain respectively).

Recent deep neural network based FSS methods (like \cite{AMP, PANet, SGOne, CANet}) employ variations of the following broad process (\autoref{fig:task_seg}): \begin{enumerate}  
\item Query and support image features are extracted using shared, pre-trained (on ImageNet \cite{ILSVRC15}) network layers.
\item A probe representation for regions of attention in the support image is obtained from the support features and mask(s).
\item The attention representation is fused with the query features. 
\item The fused features are decoded to the query mask.
\end{enumerate}
The attention extraction and fusion modules leverage the high-dimensional feature similarity between the query and the support images to selectively decode the query features to output the segmentation mask. The focus of this work is to demonstrate gaps in the propagation of this similarity information in existing methods and to bridge those gaps.

Experiments with two state-of-the-art methods - \cite{AMP} and \cite{CANet} (see Section \ref{secPremise}) reveal that FSS methods make errors in visually similar regions, across image pair samples of identical classes. They perform poorly for identical support and query inputs too. These results indicate that the class and visual similarity information is not propagated optimally across the support and query branches . 

We predict the support mask from the support features to endow the features with specificity with respect to the target class which in turn aids in similarity propagation between the support and query. We also leverage the similarities in the background regions of the support and query images through a background attention vector computed from the support features and mask, and fused with the query features. Finally, to prevent the network from over-fitting on training class-conditional similarities, we employ an input channel averaging input augmentation for the query input. With these improvements we achieve state-of-the-art performance on PASCAL $5^i$ dataset for both one-shot and five-shot segmentation tasks. 

To summarize, the paper makes the following contributions:
\begin{enumerate}[nosep]
\item A new state-of-the-art few-shot segmentation framework.
\item A dual-prediction scheme (DPr) where both the query and support masks are predicted using the same decoder.
\item A foreground-background attentive fusion mechanism for better utilization of background region similarities between the query and support images.
\item An input channel averaging regularization for preventing over-fitting on the training classes.
\end{enumerate}

\noindent  The next section places the proposed method in the context of previous work related to the problem.



==> src/introduction_pass0.tex <==
\section{Introduction}
\label{secIntro}
Semantic image segmentation assigns class labels to image pixels. It finds applications in image editing \cite{SemanticSoftSeg, Aksoy1, Aksoy2, singa, Tai, Tan}, medical diagnosis \cite{UNet, AttentionUL, HyperDenseNetAH, MultiscaleGA}, automated driving \cite{Cordts_2016_CVPR} etc. Supervised deep neural network methods such as \cite{DeepHR, SegNet, dlv1, dlv2, DLV3, dlv3plus, psp} enable highly accurate image segmentation. However, they work for only a small number of fixed object classes, and require a large number of image-mask pairs for training which are hard to manually annotate. Few-shot image segmentation methods, like \cite{OSLFSS, CANet, PANet}, are class-agnostic and alleviate the need for large number of annotated data for each target object class. They use a small set of \textit{support} images and their segmentation masks for the target class as additional input to predict the segmentation mask of a given image. 
\begin{figure}[t]
\begin{center}
    \centering
    \includegraphics[width=\linewidth]{src/images/FewshotSeg4.png}
\end{center}
\vspace{-4mm}
    \caption{Few-shot Image Segmentation: Broad architecture of contemporary state-of-the-art networks (\cite{PANet, SGOne, CANet}). Features from the support image (in the region corresponding to the support mask) are processed to obtain a probe representation and fused with features from the query image, and decoded to predict the query mask. Carrying similarity information from the support image features to the query branch is the focus of this work.}
    \label{fig:task_seg}
\end{figure}
In this paper, we analyze gaps in existing few-shot segmentation methods, and propose a method that significantly improves upon the state-of-the-art.

Few-shot segmentation (FSS) methods typically have three kinds of input - a \textit{query} image, a set of  \textit{support} images and their segmentation masks (\textit{support masks}) - from which they learn to predict the segmentation mask for the query image. The setting with a single support image and mask is termed one-shot segmentation. Our method achieves state-of-the-art performance in both one-shot ($>$5\% gain), and few-shot ($>$6.5\% gain) settings.

Recent deep neural network based methods for few-shot segmentation (like \cite{AMP, PANet, SGOne, CANet}) employ variations of the following broad process (\autoref{fig:task_seg}): \begin{enumerate}  
\item Query and support image features are extracted using shared, pre-trained network layers.
\item A probe representation for regions of attention in the support image is obtained from the support features and mask(s).
\item The attention representation is fused with the query features. 
\item The fused features are decoded to the query mask.
\end{enumerate}
The attention extraction and fusion modules leverage the high-dimensional feature similarity between the query and the support images to selectively decode the query features to output the segmentation mask. The focus of this work is to demonstrate gaps in the propagation of this similarity information in existing methods, and to bridge those gaps.

Our premise that gaps exist in similarity propagation in current methods is based on experiments with two state-of-the-art methods - \cite{CANet} and \cite{AMP} (see Section \ref{secPremise}). We find that both methods make errors in visually similar regions, across image pair samples of identical classes. They perform poorly for identical support and query inputs too. These results indicate that the class and visual similarity information is not propagated optimally across the support and query branches . 

We posit that the features employed for extracting the support representation from the support image, lack specificity and cannot be used to recover back even the support mask. To fix this problem, we propose to predict the support mask from the same modules that are used for predicting the query mask. This is achieved by fusing the support features with the attention vector and then decoding them using the query mask decoder. Next, we propose to leverage the similarities in the background pixels of the support and query images through a dual attentive fusion module. This module computes an inverse attention vector from the background regions of the support image and fuses them with the query features. Finally, to prevent the network from over-fitting on training class-conditional similarities, we propose to employ a channel averaging input augmentation for the query input. Building over the Atrous Spatial Pyramid Pooling network (introduced in \cite{dlv2}) and used by \cite{CANet}), we construct our network \textit{SimPropNet}. With these improvements we achieve state-of-the-art performance on PASCAL $5^i$ dataset for both one-shot and five-shot segmentation tasks. 

To summarize, the paper makes the following contributions:
\begin{enumerate}[nosep]
    \item A detailed analysis of the gaps in similarity propagation in few-shot segmentation methods.  
    \item A dual-prediction scheme where both the query and support masks are predicted using the same decoder.
    \item A dual attentive fusion mechanism for better utilization of background pixel similarities between the query and support images.
\end{enumerate}

We show that our the proposed approach achieves state-of-the-art performance on the PASCAL-$5^i$ dataset for both the one-shot as well as few-shot setting.

\noindent  The next section places the proposed method in the context of previous work related to the problem.



==> src/tables/fg_bg_metric.tex <==
\begin{table}[!htbp]
\centering
%\resizebox{\linewidth}{!}{
\small
\begin{tabular}{ c | c c}
\toprule
Method & 1-shot & 5-shot \\

\cmidrule(lr){1-3}

						
SimPropNet(ours) & \textbf{72.96}  & \textbf{ 72.90}\\

FWB \cite{FWB} & - & - \\

PGN \cite{PGN19} & 69.9 & 70.5 \\

PA-Net \cite{PANet} & 66.5 & 70.7 \\

CA-Net \cite{CANet} & 66.2 & 69.6 \\

SG-One \cite{SGOne} & 63.1 & 65.9\\

AMP \cite{AMP} & 62.2 & 63.8\\

OSLSM \cite{OSLFSS} & 61.3 & 61.5\\

co-FCN \cite{CoFCN} & 60.1 & 60.2\\


 \bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{Comparison tables with the FG-BG metric as used in \cite{CoFCN} for the 1-shot and 5-shot setting.}
% \vspace*{-3mm}
\label{tab:fg_bg}
\end{table}

% Overall: FG BG
% One Shot: 73.11 (55.88, 90.33); 79.23 (69.57, 88.89); 62.62 (42.65, 82.59); 76.86 (62.1, 91.64) = 72.96

% Few Shot: 74.21 (57.83, 90.59), 79.20 (69.67, 88.73), 65.23(46.7, 83.69), 71.57 (57.1, 85.9) = 72.90

==> src/tables/nullsupport_ca.tex <==
\begin{table}[!htbp]
\centering
% \resizebox{\textwidth}{!}{
%\small
\begin{tabular}{p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}}
\toprule
	& Split-1 & Split-2 & Split-3 & Split-4 \\
\toprule
$SM\neq0$ & 51.17  & 61.4 & & \\
$SM=0$ & 51.64 & 62.40 & & \\
\midrule
$\Delta mIoU$ &  & & &  \\
\bottomrule
\end{tabular}
\vspace{-0.2mm}
\caption{Drop in mean IoU Performance of CANet \cite{CANet} with null support.}
\label{tab:nullSupport}
\end{table}

==> src/tables/support_eq_query_before_after.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{p{0.18\linewidth}|p{0.11\linewidth}|p{0.11\linewidth}|p{0.11\linewidth}|p{0.11\linewidth}|p{0.11\linewidth}}
    \toprule
    Method & split-1 & split-2 & split-3 & split-4 & mean \\
    \toprule
    SimPropNet & 71.24 & 82.09 & 74.97 & 77.15 & 76.36 \\
    CANet & 54.51 &	63.98 &	48.2 &	52.76  & 54.86\\
    AMP & 54.41 &	69.34 &	64.79 &	60.02  & 62.14\\
    \midrule
    $\Delta$CANet & 16.73 & 18.11 & 26.77 & 24.39 & 21.5 \\
    $\Delta$AMP &  16.83 & 12.75 & 10.18 & 17.13 & 14.23 \\
    \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \caption{Percentage (\%) mean-IoU measured for FSS methods as compared with the proposed SimPropNet for test images from PASCAL $5^i$ dataset when query image ($I_{q}$) = support image ($I_{s}$) }
    \label{tab:sameImage_before_after}
\end{table}

==> src/tables/support_mask_zero_before_after.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{p{0.22\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}}
    \toprule
    FSS Method & Split 1 & Split 2 & Split 3 & Split 4 \\
    \toprule
    SimPropNet & & & & \\
    $M_s\neq0$ & 54.86  & 67.33 & 54.52 & 52.02  \\
    $M_s=0$ & 24.71 & 6.7 & 27.73 & 12.91 \\
    $\Delta M_s$ & \textbf{30.15\%} & \textbf{60.63\%} & \textbf{26.79\%} &  \textbf{39.11\%}\\
    \midrule
    CANet & & & & \\
    $M_s\neq0$ & 50.41\% & 63.02\% & 46.09\% & 47.46\% \\
    $M_s=0$ & 38.16\%  & 25.21\% & 27.02\% & 38.91\% \\
    $\Delta M_s$ & 12.25\% & 37.81\% & 19.07\% & 8.55\% \\
    \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \caption{Mean-IoU measured for OSS methods with support mask = 0 for test images from PASCAL $5^i$ dataset as compared with proposed SimPropNet.}
    \label{tab:nosupport_before_after}
\end{table}

==> src/tables/update_comp.tex <==
\begin{table*}[!htbp]
\centering
% \resizebox{\textwidth}{!}{
%\small
\begin{tabular}{ c | c c c c c | c c c c c}
\toprule
Method & & & 1-shot & & & & & 5-shot & & \\

\cmidrule(lr){2-6}
\cmidrule(lr){7-11}

& split-1 & split-2 & split-3 & split-4	& mean & split-1 & split-2 & split-3 & split-4	& mean \\
\cmidrule(lr){1-1}
\cmidrule(lr){2-6}
\cmidrule(lr){7-11}
						
SimPropNet(ours) & 54.86  & \textbf{67.33} & 54.52 & 52.02 & \textbf{57.19} & 57.20 & \textbf{68.50} & 58.40 & \textbf{56.05} & \textbf{60.04}  \\

FWB \cite{FWB} & 51.30 & 64.49 & \textbf{56.71} & \textbf{52.24} & 56.19 & 54.84 & 67.38 & \textbf{62.16} & 55.30 & 59.92 \\

PGN \cite{PGN19} & \textbf{56.00} & 66.90 & 50.60 & 50.40 & 56.00 & \textbf{57.70} & 67.70 & 52.90 & 54.60 & 58.50 \\

CA-Net \cite{CANet} & 50.41 & 63.02 & 46.09 & 47.46 & 51.75 & 52.27 & 65.29 & 47.15 & 50.50 & 53.81  \\

PA-Net \cite{PANet} & 42.40 & 58.00 & 51.10 & 41.20 & 48.13 & 51.80 &   64.60 & 59.80 & 46.50 & 55.70 \\

SG-One \cite{SGOne} & 40.20 & 58.40 & 48.40 & 38.40 & 46.30 & 41.90 & 58.60 & 48.60 & 39.40 & 47.10 \\

AMP \cite{AMP} & 41.90 & 50.20 & 46.70 & 34.70 & 43.40 & 41.80 & 55.50 & 50.30 & 39.90 & 46.90 \\

co-FCN \cite{CoFCN} & 36.70 & 50.60 & 44.90 & 32.40 & 41.10 & 37.50 & 50.00 & 44.10 & 33.90 & 41.40 \\

OSLSM \cite{OSLFSS} & 33.60 & 55.30 & 40.90 & 33.50 & 40.80 &35.90 & 58.10 & 42.70 & 39.10 & 43.90 \\

%AMP \cite{AMP} & 35.20 & 45.70 & 39.30 & 34.20 & 38.60  \\

 \bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{Percentage (\%) mean-IoU of one-shot segmentation on the PASCAL $5^i$ dataset using random partitions. The best results are highlighted in bold. SimProp-Net achieves state-of-the-art performance on both the 1-shot and 5-shot settings.}
% \vspace*{-3mm}
\label{tab:ret_map}
\end{table*}
